A Sharp Free Surface Finite Volume Method Applied to Gravity Wave Flows

This paper presents a sharp free surface method for fully nonlinear flow of two immiscible phases for wave propagation problems in the Finite Volume framework. The method resolves a sharp interface between two phases by combining the geometric reconstruction Volume-of-Fluid scheme isoAdvector for accurate advection of the free surface with the Ghost Fluid Method for the consistent treatment of density and pressure gradient discontinuities at the free surface. The method uses a compact computational stencil irrespective of cell shape and is formally second-order accurate in time and space. The primary focus of this work is to present the combined method and verify and validate it for wave-related problems in ocean sciences, marine and coastal engineering, by considering the following test cases: i) wave propagation of a two-dimensional wave with moderate steepness, ii) green water (water-on-deck) simulations for a ship model with violent free surface flow patterns. The method is implemented in OpenFOAM, an open source software for Computational Fluid Dynamics.

==> packagesAndStyles/tex/doc/latex/l3kernel/README <==
LaTeX3 Programming Conventions
==============================

Overview
--------

The files of the `l3kernel` bundle provide a low-level API for TeX programmers
with special syntax conventions, completely separating it from document level
syntax. Hence, the commands provided are not intended for use at the document
level nor for use in describing design layouts in document class files.

This API provides the foundation on which the LaTeX3 kernel and other advanced
extensions are built. Special care has been taken so that they can be used
within a LaTeX2e context as regular packages.

While `l3kernel` is still experimental, the bundle is now regarded as broadly
stable. The syntax conventions and functions provided are now ready for wider
use. There may still be changes to some functions, but these will be minor when
compared to the scope of `l3kernel`.

Programmers making use of `l3kernel` are *strongly* encouraged to subscribe to
the LaTeX-L mailing list (see below): announcements concerning the deprecation
or modification of functions are made on the list.

Requirements
------------

The `l3kernel` bundle requires the e-TeX extensions and the functionality
of the `\pdfstrcmp` primitive. As a result, the bundle will only work
with the following engines:

 - pdfTeX v1.30 or later
 - XeTeX v0.9994 or later
 - LuaTeX v0.40 or later

pdfTeX v1.30 was released in 2005, and so any recent TeX distribution
will support `l3kernel`. Both XeTeX and LuaTeX have developed more
actively over the past few years, and for this reason only recent
releases of these engines are supported.

Discussion
----------

Discussion concerning the approach, suggestions for improvements,
changes, additions, _etc._ should be addressed to the list
[LaTeX-L](http://news.gmane.org/group/gmane.comp.tex.latex.latex3).

You can subscribe to this list by sending mail to

  listserv@urz.uni-heidelberg.de

with the body containing

  subscribe LATEX-L  <Your-First-Name> <Your-Second-Name>

Bugs
----

The issue tracker for LaTeX3 bugs is currently located at

  https://github.com/latex3/svn-mirror/issues

Please report specific issues with LaTeX3 code there. More general
discussion should be directed to the LaTeX-L lists.

The LaTeX3 Project
------------------

Development of LaTeX3 is carried out by
[The LaTeX3 Project](http://www.latex-project.org/latex3.html). Currently,
the team members are

  * Johannes Braams
  * David Carlisle
  * Robin Fairbairns
  * Bruno Le Floch
  * Thomas Lotze
  * Frank Mittelbach
  * Will Robertson
  * Chris Rowley
  * Rainer Schöpf
  * Joseph Wright

Former members of The LaTeX3 Project team were

  * Michael Downes
  * Denys Duchier
  * Morten Høgholm
  * Alan Jeffrey
  * Martin Schröder

The development team can be contacted
by e-mail: <latex-team@latex-project.org>; for general LaTeX3 discussion
the [LaTeX-L list](http://news.gmane.org/group/gmane.comp.tex.latex.latex3)
should be used.

-----

Copyright (C) 1998-2012 The LaTeX3 Project
All rights reserved

==> packagesAndStyles/tex/doc/latex/l3kernel/source3body.tex <==
% \iffalse meta-comment
%
%% File: source3body.tex Copyright (C) 1990-2012 The LaTeX3 Project
%%
%% It may be distributed and/or modified under the conditions of the
%% LaTeX Project Public License (LPPL), either version 1.3c of this
%% license or (at your option) any later version.  The latest version
%% of this license is in the file
%%
%%    http://www.latex-project.org/lppl.txt
%%
%% This file is part of the "l3kernel bundle" (The Work in LPPL)
%% and all files in that bundle must be distributed together.
%%
%% The released version of this bundle is available from CTAN.
%%
%% -----------------------------------------------------------------------
%%
%% The development version of the bundle can be found at
%%
%%    http://www.latex-project.org/svnroot/experimental/trunk/
%%
%% for those people who are interested.
%%
%%%%%%%%%%%
%% NOTE: %%
%%%%%%%%%%%
%%
%%   Snapshots taken from the repository represent work in progress and may
%%   not work or may contain conflicting material!  We therefore ask
%%   people _not_ to put them into distributions, archives, etc. without
%%   prior consultation with the LaTeX3 Project.
%%
%% -----------------------------------------------------------------------
%
% \fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% This file is used by
%
%  source3.tex            % documentation including implementation
%
%  interface3.tex         % only interface documentation
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{abstract}

\setlength\parindent{0pt}
\setlength\parskip{\baselineskip}

\noindent
This is the reference documentation for the \pkg{expl3}
programming environment. The \pkg{expl3} modules set up an experimental
naming scheme for \LaTeX{} commands, which allow the \LaTeX{} programmer
to systematically name functions and variables, and specify the argument
types of functions.

The \TeX{} and \eTeX{} primitives are all given a new name according to
these conventions. However, in the main direct use of the primitives is
not required or encouraged: the \pkg{expl3} modules define an
independent low-level \LaTeX3 programming language.

At present, the \pkg{expl3} modules are designed to be loaded on top of
\LaTeXe{}. In time, a \LaTeX3 format will be produced based on this code.
This allows the code to be used in \LaTeXe{} packages \emph{now} while a
stand-alone \LaTeX3 is developed.

\begin{bfseries}
  While \pkg{expl3} is still experimental, the bundle is now regarded as
  broadly stable. The syntax conventions and functions provided are now
  ready for wider use. There may still be changes to some functions, but
  these will be minor when compared to the scope of \pkg{expl3}.

  New modules will be added to the distributed version of \pkg{expl3} as
  they reach maturity.
\end{bfseries}

\end{abstract}

\clearpage

{%
  \def\\{:}% fix "newlines" in the ToC
  \tableofcontents
}

\clearpage
\pagenumbering{arabic}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Each of the following \DocInput lines includes a file with extension
% .dtx. Each of these files may be typeset separately. For instance
%   pdflatex l3box.dtx
% will typeset the source of the LaTeX3 box commands. If you use the
% Makefile, the index will be generated automatically; e.g.,
%   make doc F=l3box
%
% If this file is processed, each of these separate dtx files will be
% contained as a part of a single document.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter
\def\partname{Part}
\def\maketitle{\clearpage\part{\@title}}
\let\thanks\@gobble
\let\DelayPrintIndex\PrintIndex
\let\PrintIndex\@empty
\makeatother

\part{Introduction to \pkg{expl3} and this document}

This document is intended to act as a comprehensive reference manual
for the \pkg{expl3} language. A general guide to the \LaTeX3
programming language is found in \href{expl3.pdf}{expl3.pdf}.

\section{Naming functions and variables}

\LaTeX3 does not use \texttt{@} as a \enquote{letter} for defining
internal macros.  Instead, the symbols |_| and \texttt{:}
are used in internal macro names to provide structure. The name of
each \emph{function} is divided into logical units using \texttt{_},
while \texttt{:} separates the \emph{name} of the function from the
\emph{argument specifier} (\enquote{arg-spec}). This describes the arguments
expected by the function. In most cases, each argument is represented
by a single letter. The complete list of arg-spec letters for a function
is referred to as the \emph{signature} of the function.

Each function name starts with the \emph{module} to which it belongs.
Thus apart from a small number of very basic functions, all \pkg{expl3}
function names contain at least one underscore to divide the module
name from the descriptive name of the function. For example, all
functions concerned with comma lists are in module \texttt{clist} and
begin \cs{clist_}.

Every function must include an argument specifier. For functions which
take no arguments, this will be blank and the function name will end
\texttt{:}. Most functions take one or more arguments, and use the
following argument specifiers:
\begin{description}
  \item[\texttt{D}] The \texttt{D} specifier means \emph{do not use}.
    All of the \TeX{} primitives are initially \cs{let} to a \texttt{D}
    name, and some are then given a second name.  Only the kernel
    team should use anything with a \texttt{D} specifier!
  \item[\texttt{N} and \texttt{n}] These mean \emph{no manipulation},
    of a single token for \texttt{N} and of a set of tokens given in
    braces for \texttt{n}. Both pass the argument through exactly as
    given. Usually, if you use a single token for an \texttt{n} argument,
    all will be well.
  \item[\texttt{c}] This means \emph{csname}, and indicates that the
    argument will be turned into a csname before being used. So
    So \cs{foo:c} |{ArgumentOne}| will act in the same way as \cs{foo:N}
    \cs{ArgumentOne}.
  \item[\texttt{V} and \texttt{v}] These mean \emph{value
    of variable}. The \texttt{V} and \texttt{v} specifiers are used to
    get the content of a variable without needing to worry about the
    underlying \TeX{} structure containing the data. A \texttt{V}
    argument will be a single token (similar to \texttt{N}), for example
    \cs{foo:V} \cs{MyVariable}; on the other hand, using \texttt{v} a
    csname is constructed first, and then the value is recovered, for
    example \cs{foo:v} |{MyVariable}|.
  \item[\texttt{o}] This means \emph{expansion once}. In general, the
    \texttt{V} and \texttt{v} specifiers are favoured over \texttt{o}
    for recovering stored information. However, \texttt{o} is useful
    for correctly processing information with delimited arguments.
  \item[\texttt{x}] The \texttt{x} specifier stands for \emph{exhaustive
    expansion}: every token in the argument is fully expanded until only
    unexpandable ones remain. The \TeX{} \tn{edef} primitive carries out
    this type of expansion. Functions which feature an \texttt{x}-type
    argument are in general \emph{not} expandable, unless specifically
    noted.
  \item[\texttt{f}] The \texttt{f} specifier stands for \emph{full
    expansion}, and in contrast to \texttt{x} stops at the first
    non-expandable item (reading the argument from left to right) without
    trying to expand it. For example, when setting a token list
    variable (a macro used for storage), the sequence
    \begin{verbatim}
      \tl_set:Nn \l_mya_tl { A }
      \tl_set:Nn \l_myb_tl { B }
      \tl_set:Nf \l_mya_tl { \l_mya_tl \l_myb_tl }
    \end{verbatim}
    will leave |\l_mya_tl| with the content |A\l_myb_tl|, as |A| cannot
    be expanded and so terminates expansion before |\l_myb_tl| is considered.
  \item[\texttt{T} and \texttt{F}] For logic tests, there are the branch
    specifiers \texttt{T} (\emph{true}) and \texttt{F} (\emph{false}).
    Both specifiers treat the input in the same way as \texttt{n} (no
    change), but make the logic much easier to see.
  \item[\texttt{p}] The letter \texttt{p} indicates \TeX{}
    \emph{parameters}. Normally this will be used for delimited
    functions as \pkg{expl3} provides better methods for creating simple
    sequential arguments.
  \item[\texttt{w}] Finally, there is the \texttt{w} specifier for
    \emph{weird} arguments. This covers everything else, but mainly
    applies to delimited values (where the argument must be terminated
    by some arbitrary string).
\end{description}
Notice that the argument specifier describes how the argument is
processed prior to being passed to the underlying function. For example,
\cs{foo:c} will take its argument, convert it to a control sequence and
pass it to \cs{foo:N}.

Variables are named in a similar manner to functions, but begin with
a single letter to define the type of variable:
\begin{description}
  \item[\texttt{c}] Constant: global parameters whose value should not
    be changed.
  \item[\texttt{g}] Parameters whose value should only be set globally.
  \item[\texttt{l}] Parameters whose value should only be set locally.
\end{description}
Each variable name is then build up in a similar way to that of a
function, typically starting with the module\footnote{The module names are
  not used in case of generic scratch registers defined in the data
  type modules, e.g., the
  \texttt{int} module contains some scratch variables called \cs{l_tmpa_int},
  \cs{l_tmpb_int}, and so on. In such a case adding the module name up front
  to denote the module
  and in the back to indicate the type, as in
  \cs{l_int_tmpa_int} would be very unreadable.}  name
and then a descriptive part.
Variables end with a short identifier to show the variable type:
\begin{description}
  \item[\texttt{bool}] Either true or false.
  \item[\texttt{box}] Box register.
  \item[\texttt{clist}] Comma separated list.
  \item[\texttt{coffin}] a \enquote{box with handles} --- a higher-level data
     type for carrying out |box| alignment operations.
  \item[\texttt{dim}] \enquote{Rigid} lengths.
  \item[\texttt{fp}] floating-point values;
  \item[\texttt{int}] Integer-valued count register.
  \item[\texttt{prop}] Property list.
  \item[\texttt{seq}] \enquote{Sequence}: a data-type used to implement lists
    (with access at both ends) and stacks.
  \item[\texttt{skip}] \enquote{Rubber} lengths.
  \item[\texttt{stream}] An input or output stream (for reading from or
    writing to, respectively).
  \item[\texttt{tl}] Token list variables: placeholder for a token list.
\end{description}

\subsection{Terminological inexactitude}

A word of warning. In this document, and others referring to the \pkg{expl3}
programming modules, we often refer to \enquote{variables} and
\enquote{functions} as if they
were actual constructs from a real programming language.  In truth, \TeX{}
is a macro processor, and functions are simply macros that may or may not take
arguments and expand to their replacement text.  Many of the common variables
are \emph{also} macros, and if placed into the input stream will simply expand
to their definition as well~--- a \enquote{function} with no arguments and a
\enquote{token list variable} are in truth one and the same.  On the other
hand, some \enquote{variables} are actually registers that must be
initialised and their values set and retrieved with specific functions.

The conventions of the \pkg{expl3} code are designed to clearly separate the
ideas of \enquote{macros that contain data} and
\enquote{macros that contain code}, and a
consistent wrapper is applied to all forms of \enquote{data} whether they be
macros or
actually registers.  This means that sometimes we will use phrases like
\enquote{the function returns a value}, when actually we just mean
\enquote{the macro expands to something}. Similarly, the term
\enquote{execute} might be used in place of \enquote{expand}
or it might refer to the more specific case of
\enquote{processing in \TeX's stomach}
(if you are familiar with the \TeX{}book parlance).

If in doubt, please ask; chances are we've been hasty in writing certain
definitions and need to be told to tighten up our terminology.

\section{Documentation conventions}

This document is typeset with the experimental \pkg{l3doc} class;
several conventions are used to help describe the features of the code.
A number of conventions are used here to make the documentation clearer.

Each group of related functions is given in a box. For a function with
a \enquote{user} name, this might read:
\begin{function}{\ExplSyntaxOn, \ExplSyntaxOff}
  \begin{syntax}
    \cs{ExplSyntaxOn} \dots{} \cs{ExplSyntaxOff}
  \end{syntax}
  The textual description of how the function works would appear here. The
  syntax of the function is shown in mono-spaced text to the right of
  the box. In this example, the function takes no arguments and so the
  name of the function is simply reprinted.
\end{function}

For programming functions, which use \texttt{_} and \texttt{:} in their name
there are a few additional conventions: If two related functions are given
with identical names but different argument specifiers, these are termed
\emph{variants} of each other, and the latter functions are printed in grey to
show this more clearly. They will carry out the same function but will take
different types of argument:
\begin{function}{\seq_new:N, \seq_new:c}
  \begin{syntax}
    \cs{seq_new:N} \meta{sequence}
  \end{syntax}
  When a number of variants are described, the arguments are usually
  illustrated only for the base function. Here, \meta{sequence} indicates
  that \cs{seq_new:N} expects the name of a sequence. From the argument
  specifier, \cs{seq_new:c} also expects a sequence name, but as a
  name rather than as a control sequence. Each argument given in the
  illustration should be described in the following text.
\end{function}

\paragraph{Fully expandable functions}
\hypertarget{expstar}{Some functions are fully expandable},
which allows it to be used within
an \texttt{x}-type argument (in plain \TeX{} terms, inside an \cs{edef}),
as well as within an \texttt{f}-type argument.
These fully expandable functions are indicated in the documentation by
a star:
\begin{function}[EXP]{\cs_to_str:N}
  \begin{syntax}
    \cs{cs_to_str:N} \meta{cs}
  \end{syntax}
  As with other functions, some text should follow which explains how
  the function works. Usually, only the star will indicate that the
  function is expandable. In this case, the function expects a \meta{cs},
  shorthand for a \meta{control sequence}.
\end{function}

\paragraph{Restricted expandable functions}
\hypertarget{rexpstar}{A few functions are fully expandable} but cannot be fully expanded within
an \texttt{f}-type argument. In this case a hollow star is used to indicate
this:
\begin{function}[rEXP]{\seq_map_function:NN}
  \begin{syntax}
    \cs{seq_map_function:NN} \meta{seq} \meta{function}
  \end{syntax}
\end{function}

\paragraph{Conditional functions}
\hypertarget{explTF}{Conditional (\texttt{if}) functions}
are normally defined in three variants, with
\texttt{T}, \texttt{F} and \texttt{TF} argument specifiers. This allows
them to be used for different \enquote{true}/\enquote{false} branches,
depending on
which outcome the conditional is being used to test. To indicate this
without repetition, this information is given in a shortened form:
\begin{function}[EXP,TF]{\xetex_if_engine:}
  \begin{syntax}
    \cs{xetex_if_engine:TF} \Arg{true code} \Arg{false code}
  \end{syntax}
  The underlining and italic of \texttt{TF} indicates that
  \cs{xetex_if_engine:T}, \cs{xetex_if_engine:F} and
  \cs{xetex_if_engine:TF} are all available. Usually, the illustration
  will use the \texttt{TF} variant, and so both \meta{true code}
  and \meta{false code} will be shown. The two variant forms \texttt{T} and
  \texttt{F} take only \meta{true code} and \meta{false code}, respectively.
  Here, the star also shows that this function is expandable.
  With some minor exceptions, \emph{all} conditional functions in the
  \pkg{expl3} modules should be defined in this way.
\end{function}

Variables, constants and so on are described in a similar manner:
\begin{variable}{\l_tmpa_tl}
  A short piece of text will describe the variable: there is no
  syntax illustration in this case.
\end{variable}

In some cases, the function is similar to one in \LaTeXe{} or plain \TeX{}.
In these cases, the text will include an extra \enquote{\textbf{\TeX{}hackers
note}} section:
\begin{function}[EXP]{\token_to_str:N}
  \begin{syntax}
    \cs{token_to_str:N} \meta{token}
  \end{syntax}
  The normal description text.
  \begin{texnote}
    Detail for the experienced \TeX{} or \LaTeXe\ programmer. In this
    case, it would point out that this function is the \TeX{} primitive
    \cs{string}.
  \end{texnote}
\end{function}

\section{Formal language conventions which apply generally}

As this is a formal reference guide for \LaTeX3 programming, the descriptions
of functions are intended to be reasonably \enquote{complete}. However, there
is also a need to avoid repetition. Formal ideas which apply to general
classes of function are therefore summarised here.

For tests which have a \texttt{TF} argument specification, the test if
evaluated to give a logically \texttt{TRUE} or \texttt{FALSE} result.
Depending on this result, either the \meta{true code} or the \meta{false code}
will be left in the input stream. In the case where the test is expandable,
and a predicate (|_p|) variant is available, the logical value determined by
the test is left in the input stream: this will typically be part of a larger
logical construct.

\section{\TeX{} concepts not supported by \LaTeX3{}}

The \TeX{} concept of an \enquote{\cs{outer}} macro is \emph{not supported}
at all by \LaTeX3{}. As such, the functions provided here may break when
used on top of \LaTeXe{} if \cs{outer} tokens are used in the arguments.

\DisableImplementation

\DocInput{l3bootstrap.dtx}
\DocInput{l3names.dtx}
\DocInput{l3basics.dtx}
\DocInput{l3expan.dtx}
\DocInput{l3prg.dtx}
\DocInput{l3quark.dtx}
\DocInput{l3token.dtx}
\DocInput{l3int.dtx}
\DocInput{l3skip.dtx}
\DocInput{l3tl.dtx}
\DocInput{l3seq.dtx}
\DocInput{l3clist.dtx}
\DocInput{l3prop.dtx}
\DocInput{l3box.dtx}
\DocInput{l3coffins.dtx}
\DocInput{l3color.dtx}
\DocInput{l3msg.dtx}
\DocInput{l3keys.dtx}
\DocInput{l3file.dtx}
\DocInput{l3fp.dtx}
% To get the various submodules of l3fp to appear in the implementation
% part only, they have to be added to the documentation list after typesetting
% the 'user' part just for the main module.
\ExplSyntaxOn
\clist_gput_right:Nn \g_docinput_clist
  {
    l3fp-aux.dtx ,
    l3fp-traps.dtx ,
    l3fp-round.dtx ,
    l3fp-parse.dtx ,
    l3fp-logic.dtx ,
    l3fp-basics.dtx ,
    l3fp-extended.dtx ,
    l3fp-expo.dtx ,
    l3fp-trig.dtx ,
    l3fp-convert.dtx ,
    l3fp-assign.dtx ,
    l3fp-old.dtx ,
  }
\ExplSyntaxOff
\DocInput{l3luatex.dtx}

\DocInput{l3candidates.dtx}
\DocInput{l3drivers.dtx}

\endinput


==> packagesAndStyles/tex/doc/latex/l3packages/README <==
LaTeX3 High-Level Concepts
==========================

Overview
--------

The `l3packages` collection is contains implementations for aspects of the
LaTeX3 kernel, dealing with higher-level ideas such as the Designer Interface.
The packages here are considered broadly stable (The LaTeX3 Project does not
expect the interfaces to alter radically). These packages are build on LaTeX2e
conventions at the interface level, and so may not migrate in the current form
to a stand-alone LaTeX3 format.

All of the material in the collection requires the LaTeX3 base layer package
[`l3kernel`](http://ctan.org/pkg/l3kernel). The two packages must be installed
in matching versions: if you update l3packages, make sure that `l3kernel` is
updated at the same time.

Currently included in the CTAN release of `l3packages` are the following
bundles:
 * `l3keys2e`
 * `xfrac`
 * `xparse`
 * `xtemplate`

`l3keys2e`
----------

The `l3keys2e` package allows keys defined using `l3keys` to be used as package
and class options with LaTeX2e. This is tied to the method the existing kernel
uses for processing options, and so it is likely that a stand-alone LaTeX3
kernel will use a very different approach.

`xfrac`
-------

The `xfrac` package uses the interface defined by `xtemplate` to provide
flexible split-level fractions _via_ the `\sfrac` macro. This is both a
demonstration of the power of the template concept and also a useful addition
to the available functionality in LaTeX2e.

`xparse`
-------

The `xparse` package provides a high-level interface for declaring document
commands, e.g., a uniform way to define commands taking optional arguments,
optional stars (and others), mandatory arguments and more.

`xtemplate`
-----------

The `xtemplate` package provides an interface for defining generic
functions using a key=val syntax. This is designed to be
"self-documenting", with the key definitions providing information
on how they are to be used.

Discussion
----------

Discussion concerning the approach, suggestions for improvements,
changes, additions, _etc._ should be addressed to the list
[LaTeX-L](http://news.gmane.org/group/gmane.comp.tex.latex.latex3).

You can subscribe to this list by sending mail to

  listserv@urz.uni-heidelberg.de

with the body containing

  subscribe LATEX-L  <Your-First-Name> <Your-Second-Name>

Bugs
----

The issue tracker for LaTeX3 bugs is currently located at

  https://github.com/latex3/svn-mirror/issues

Please report specific issues with LaTeX3 code there. More general
discussion should be directed to the LaTeX-L lists.

The LaTeX3 Project
------------------

Development of LaTeX3 is carried out by
[The LaTeX3 Project](http://www.latex-project.org/latex3.html). Currently,
the team members are

  * Johannes Braams
  * David Carlisle
  * Robin Fairbairns
  * Morten Høgholm
  * Bruno Le Floch
  * Thomas Lotze
  * Frank Mittelbach
  * Will Robertson
  * Chris Rowley
  * Rainer Schöpf
  * Joseph Wright

Former members of The LaTeX3 Project team were

  * Michael Downes
  * Denys Duchier
  * Alan Jeffrey
  * Martin Schröder

The development team can be contacted
by e-mail: <latex-team@latex-project.org>; for general LaTeX3 discussion
the [LaTeX-L list](http://news.gmane.org/group/gmane.comp.tex.latex.latex3)
should be used.

--- Copyright 1998-2011
    The LaTeX3 Project.  All rights reserved ---

==> packagesAndStyles/tex/doc/latex/media9/ChangeLog <==
2014-03-25
	* v0.43
	* fix: bugs related to AcroForm and OCProperties catalog entries;
	documenation

2014-03-21
	* v0.42
	* change: refined look for the play button overlay
	* fix: minor bugs

2014-03-06
	* v0.41
	* new: poster text, if provided, also shown in draft mode (instead of draft
	box)
	* new: updated VPlayer with `autoRewind' setting via FlashVars

2014-02-17
	* v0.40
	* new: play button visible in AR only
	* new: updated APlayer and VPlayer with new exposed ActionScript functions
	`currentTime', `duration', `playing', `muted'

2014-02-06
	* v0.39
	* fix: improved compatibility with `animate' package

2013-12-04
	* v0.38
	* fix: bugs in 3Dmenu

2013-11-27
	* v0.37
	* fix: error in case of control sequence used in the last argument of
	\includemedia

2013-11-26
	* v0.36
	* fix: Postscript error with zero size media annotations
	* change: updated 3Dmenu.js, transformation of mesh group nodes now possible

2013-11-15
	* v0.35
	* new: play button overlay, can be disabled with new option `noplaybutton'
	* change: updated media players

2013-11-12
	* v0.34
	* fix: `bigfiles' option and really big files caused dvips error

2013-11-04
	* new: media player Flash components VPlayer9.swf, APlayer9.swf added
	for compatibility with the Flash Player 9 plugin that is bundled with
	Adobe Reader 9.4.1 for Linux

2013-09-24
	* v0.33
	* fix: Adobe Reader prompting for "save changes" on closing

2013-09-06
	* v0.32
	* change: `bigfiles' package option no longer requires `-dNOSAFER' with
	ps2pdf.

2013-08-26
	* v0.31
	* fix: expl3 related fix for correct 3D views file processing

2013-08-16
	* v0.30
	* change: update to current expl3 version

2013-07-19
	* v0.29
	* change: minor improvements of media buttons

2013-06-07
	* fix: VPlayer updated

2013-06-06
	* fix: APlayer & VPlayer updated, all players recompiled using
	ApacheFlexSDK-4.9.1

2013-06-03
	* v0.28
	* fix: updated APlayer.swf
	* new: options `draft' and `final' for media bottons

2013-03-27
	* new: APlayer displays ID3 tags (artist, song, album), if available

2013-03-20
	* v0.26
	* new: specifier for floating window position on screen, default is centred
	* v0.27
	* fix: package option `windowed' did not work

2013-03-08
	* v0.25
	* change: VPlayer.swf with transparent background; floating media window
	now centred

2013-02-21
	* v0.24
	* change: option `url' now deprecated

2013-02-12
	* v0.23
	* change: minor usability improvements

2013-01-31
	* v0.22
	* new: user command \mediabutton for creating media control buttons

2013-01-23
	* v0.21
	* fix: swf media inserted after a 3D object didn't work, reported by C.
	Sturm

2013-01-21
	* v0.20
	* new: `hideBar' option (FlashVar) for APlayer.swf

2013-01-07
	* v0.19
	* fix: default window size calculation for floating media window

2012-12-21
	* v0.18
	* new: playback in floating window; VPlayer.swf can be configured for
	stepping mode

2012-11-26
	* v0.17
	* change: updated APlayer.swf with transparent background; poster is now inserted
	into the page content stream, not in the appearance dictionary

2012-11-20
	* v0.16
	* fix: `transparent' option now working with Flash content, updated
	StrobeMediaPlayback.swf (OSMF-2.0)

2012-10-04
	* v0.15
	* fix: error in case of multiple use of `3Dviews' option

2012-10-02
	* v0.14
	* new: keyboard control added to VPlayer.swf and APlayer.swf

2012-09-12
	* v0.13
	* fix: cross section related bug in 3Dmenu.js
	* fix: asylabels.js with improved label control (requires asymptote-2.17)

2012-09-07
	* v0.12
	* new: command option `3Dpsob' and 3d views file entry `PSOB' added on
	request	of J. Bowman (Asymptote)
	* fix: empty option list of \includemedia led to crash, improved Asymptote
	compatibility

2012-08-14
	* v0.11
	* new: package option `bigfiles' added which defers file embedding to the
	ps->pdf step; needed when latex aborts with error `TeX capacity exceeded'
	* fix: minor fixes in 3Dmenu.js and media9.sty

2012-07-31
	* v0.9, v.10
	* fix: new l3fp infix syntax for calculations; deprecated expl3 functions
	replaced

2012-07-24
	* v0.8
	* fix: changed behaviour of \fp_use:N (l3fp package) caused failure;
	opening 3D views file lead to error due to changed behaviour of
	\ior_open:Nn (l3file package)

2012-05-02
	* v0.7
	* new: 3Dpartsattrs added as package option

2012-04-25
	* v0.6
	* new: command options added: 3Dpartsattrs, label;
	updated APlayer and VPlayer versions with exposed ActionScript functions
	for player control from JavaScript

2012-04-16
	* v0.5
	* fix: option 3Dortho did not work, documentation update

2012-04-12
	* v0.4
	* new: dependency on babel package removed; code contributed by
	Enrico Gregorio
	* fix: annotation box size calculation produced non-intuitive results

2012-04-03
	* v0.3
	* fix: `deactivate' option did not work
	* new: enhanced StrobeMediaPlayback.swf video player included

2012-03-16
	* v0.2
	* new: LuaLaTeX support
	* fix: wrong poster dimension in dvi output; fp numbers in PDF objects had
	too many decimal places for dvipdfmx

2012-03-01
	* initial release (v0.1) to CTAN


==> packagesAndStyles/tex/doc/latex/media9/files/3dsystem.tex <==
\begin{picture}(0,0)%
\includegraphics[clip, scale=1, viewport=0 0 435 423.334371108344]{3dsystem}%
\end{picture}%
\setlength{\unitlength}{4144sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(6905.17992277992,6720)(435,-6602)%
\put(4471,-3469){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}{\color[rgb]{0,0,1}$\overrightarrow{C2C}$}%
}}}}%
\put(6014,-3433){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$Y$}%
}}}}%
\put(7141,-6533){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$X$}%
}}}}%
\put(2267,-458){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$Z$}%
}}}}%
\put(4091,-4976){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}{\color[rgb]{1,0,0}$\overrightarrow{COO}$}%
}}}}%
\put(2161,-5371){\makebox(0,0)[rb]{\smash{{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$(0,0,0)$}%
}}}}%
\put(2836,-1471){\makebox(0,0)[b]{\smash{{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\sphericalangle AAC$}%
}}}}%
\put(3636,-2841){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}{\color[rgb]{0,0,1}$ROO$}%
}}}}%
\end{picture}%

